RV32I in ACL2

We present a simple ACL2 simulator for the RISC-V 32-bit base instruction set architecture, written in the operational semantics style. Like many other ISA models, our RISC-V state object is a single-threaded object and we prove read-over-write, write-over-write, writing-the-read, and state well-formedness theorems. Unlike some other models, we separate the instruction decoding functions from their semantic counterparts. Accordingly, we verify encoding / decoding functions for each RV32I instruction, the proofs for which are entirely automatic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{46}
\providecommand{\publicationstatus}{Gamboa and Manolios (Eds):\\
ACL2 Workshop 2025\\
EPTCS 423, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.423.4}{10.4204/EPTCS.423.4}}
\pdfoutput=1

